VueBuds: Visual Intelligence with Wireless Earbuds

Despite their ubiquity, wireless earbuds remain audio-centric due to size and power constraints. We present VueBuds, the first camera-integrated wireless earbuds for egocentric vision, capable of operating within stringent power and form-factor limits. Each VueBud embeds a camera into a Sony WF-1000XM3 to stream visual data over Bluetooth to a host device for on-device vision language model (VLM) processing. We show analytically and empirically that while each camera's field of view is partially occluded by the face, the combined binocular perspective provides comprehensive forward coverage. By integrating VueBuds with VLMs, we build an end-to-end system for real-time scene understanding, translation, visual reasoning, and text reading; all from low-resolution monochrome cameras drawing under 5mW through on-demand activation. Through online and in-person user studies with 90 participants, we compare VueBuds against smart glasses across 17 visual question-answering tasks, and show that our system achieves response quality on par with Ray-Ban Meta. Our work establishes low-power camera-equipped earbuds as a compelling platform for visual intelligence, bringing rapidly advancing VLM capabilities to one of the most ubiquitous wearable form factors.

==> accessibility_figure_descriptions.tex <==
Figure 1
4 photos labeled (A), (B), (C), and (D) show people using IRIS to interact with various smart home devices. Image (A) shows the back of a man pointing IRIS at a smart lock to unlock his front door. Image (B) shows the back of a woman in her living room pointing IRIS at a television to control it. Image (C) shows the same woman wearing a vest, pointing at her ceiling lights to turn them on. Image (D) shows the same man from image (A) in his bedroom, pointing IRIS at a set of blinds to raise lower them.


Figure 2
This image contains two IRIS rings, IRIS printed circuit board, and a US quarter. There is a clear enclosure of IRIS showing the camera on the left along with a USB connector. The matte white IRIS ring a profile to view the button. To the right of the image is a US quarter, placed beside the assembled IRIS circuit board.


Figure 3
Graphical diagram of the IRIS system. In the center of the image, IRIS ring is shown on a user’s finger pointing at an illustration of a smart speaker in a living room. The captured image is illustrated in a green box to the right of the diagram. This image, shown as an illustration, is shown being transmitted to a phone. The image is sent to the yellow block on the right which is our neural network. The neural network (bottom right yellow box) returns the class of the object, a speaker here, and the phone issues commands to turn the speaker on.


Figure 4
Two images (A) and (B) show IRIS worn on a person’s index finger with the black camera shown. Image (A) shows a front view of the ring on a person’s hand. Image (B) shows a top down view of the ring on a person’s hand.


Figure 5
A diagram showing the data streaming pipeline of the IRIS hardware and firmware. CAM_DATA (top left corner) goes to SPIS_MOSI block, which then goes to DMA and finally arrives at an Image Buffer of 162x119 samples (light red). Similarly, IMU_DATA (bottom left corner) goes to SPIM_MISO and then DMA to arrive at an IMU Buffer (light blue) containing 256 samples. Both light red and light blue buffer go into their respective ring buffers (purple circles). The data in these ring buffers get sent to BLE Data Packer, organizing it into BLE packets as shown in the large yellow box with light blue packets. These packets then get transmitted to the final light blue block on the right (BLE 2Mbps).


Figure 6
Schematic of the IRIS neural network architecture. (1) shows a silhouette of a human and represents a user wearing IRIS. A point-and-click arrow then goes to (2) which shows a captured image from IRIS. (3) is a light red box showing YOLO, which outputs the same captured image from (2) with bounding boxes corresponding to objects it detects. Simultaneously, a light blue box (3) labeled DinoV2 outputs a Tensor of 16x16x384 which gets sent to (5). The output of (3) goes to (4) Centered Object Detection Algorithm which outputs Blinds to (5). Because there are 2 blinds in the Smart Device Library (light green box, top right), (5) outputs Blinds 2 UUID which corresponds to the 16x16x384 tensor. This gets sent to (6) Home Device Manager which controls Blinds 2. (7) shows a double-click gesture, corresponding to an undo operation. This allows users to save the most recent query as a new reference image in (5).


Table 1
Table showing the context-aware gesture set for IRIS. The table shows how the same gesture (single press or rotation) will have a different effect depending on the device (first column). For example, a rotation for lights will change the brightness, but the same gesture can also adjust the volume of a speaker. 


Figure 7
Grid of greyscale photos taken from IRIS ring showing a living room with a fan, window+blinds, and HVAC system on the wall. This figure shows how the DINOV2 query system works whereby query images (first column) are compared to reference images (rest of the columns) in the database. The reference images are ranked in decreasing order of similarity.


Figure 8
Photo of three views of the user interface for the IRIS mobile application. A camera stream from the ring is shown of a set of blinds and two ceiling lights. The second view shows smart home devices listed in a database, for a user to add reference images for. The last view shows a view to Add Device Embedding with an image of a light. The four images below this image are other reference images associated with the light.


Table 2
Table showing the IRIS ring placement preferences of the participants in the user study. The table shows participant preference for comfort, ability to target devices, and overall preference for IRIS placement on either the middle digit or proximal digit. Participants were evenly split between middle and proximal placement for comfort (p value of 0.339>0.05). Participants preferred IRIS placement on the middle digit (p value of 0.005<0.05) for ability to target devices. Participants were also fairly evenly split between middle and proximal placement in terms of overall preference (p value of 0.202>0.05).


Figure 9
Person is sitting in front of a smart speaker (left) and smart light (right). The person is pointing the IRIS ring at the smart lights and turning it on.


Figure 10
Histogram of the user survey scores for using IRIS evaluated in terms of overall experience, ease of use, and intuitiveness. Participants ranked each metric on a scale of one to five with five being the best. Scores for 1 have been omitted as no participants voted 1. A majority of participants (12) gave the overall experience a four, followed by 8 participants giving the overall experience a 5. A majority of participants (9) gave IRIS a 5 for ease of use, followed by 6 participants giving a score of 4 and another 6 giving a score of 3 for ease of use. Lastly, a majority of participants (14) gave a score of 4 for intuitiveness, followed by 6 participants giving IRIS a score of 5 for intuitiveness. 


Table 3
Table showing the participant preferences for using IRIS versus Siri for toggling device state, granular control, social acceptability, and preference for day-to-day use. Participants showed no significant leaning towards using IRIS over SIRI for toggling device state (p value 0.202 is greater than 0.05) with a majority favoring IRIS. Participants significantly favored using IRIS over SIRI for granular control (p value of 0.001 less than 0.05) and in terms of social acceptability (p value of 0.017 less than 0.05). Lastly, participants showed no significant leaning towards day to day use between IRIS or SIRI (p value 0.196 greater than 0.05) with a majority of participants (47.8%) indicating that they would use both day to day.


Figure 11
Four histograms are shown in this figure. The top two histograms show the user input to device output times across all participants in our user study (a). The bottom two histograms show time to set a desired volume across all participants in our user study (b). Both IRIS and SIRI show a positive skew for the user input to device output times. IRIS has a median user input to device output time of 2.2 seconds compared to voice with a median of 4.1 seconds. IRIS and SIRI also both show a positive skew for the time to set desired volume, with IRIS having a median time of 4.8 seconds compared to SIRI which has a median time of 7.6 seconds. 


Figure 12
Confusion matrix results across five supported smart device classes using YOLO (You only look once) and CODA (centered object detection algorithm). There is 100% prediction accuracy for blinds, smart locks, speakers, and TVs, 93% accuracy for lights, and 83% accuracy for background. Background was predicted as speaker 6% of the time, TV 6% of the time, and lights 6% of the time. Lights were predicted as background 7% of the time.


Figure 13
Line graph showing the accuracy of DINOV2 as the number of reference images for each device instance increases. For a single reference image in the database, DINO achieves an accuracy of approximately 88%. For two reference images, the accuracy increases to about 95%. For three images the accuracy increases to 98% and plateaus for additional images beyond three. 


Figure 14
A two by six grid of photos captured from the IRIS ring showing different smart locks. In the first column, two images are shown of a smart lock with the label Query. In the second column, two images of smart locks are shown with the label Prediction. And in the last four columns, seven images of smart locks are shown with the label References. The bottom row shows that by adding an additional reference image, the query accurately predicts the correct instance of the smart lock, as opposed to the top row which shows a different instance of smart lock.


Table 4
Table showing the latency breakdown across the hardware and neural network components as a function of the size of the DINOV2 embedding database size, with sizes of 4, 50, and 100 embeddings. The hardware latency is constant at 293 milliseconds at each database size.The Yolo classification latency is also constant at each database size, remaining constant at 28 milliseconds. And the embedding generation latency is also constant at 8 milliseconds at each database size. The embedding query latency increases from 9 milliseconds at a database size of 4 images, to 244 milliseconds for a database size of 50 images, to 752 milliseconds for a database size of 100 reference images. 


Figure 15
Bar chart showing the inference time for YOLO+CODA+DINO for a sample of lights (20 samples), doors (4 samples), blinds (9 samples), smart locks (10 samples), speakers (30 samples), and TV (13 samples), as well as inference time when using DINOV2 only (86 samples). The inference times for the individual classes are lower (less than 200ms) because we use the classification from YOLO+CODA to reduce the search space of DINOV2 Only (400+ms).


Table 5
Table showing the IRIS hardware power consumption by component in each operating state: SLEEP, IDLE, and ACTIVE. The estimated total power consumption for SLEEP, IDLE, and ACTIVE are 34.03 microwatts, 3.76 milliwatts, and 21.2 milliwatts respectively. The measured total power consumption for SLEEP, IDLE, and ACTIVE are 86.5 microwatts, 6.63 milliwatts, and 26.1 milliwatts, respectively. 


Table 6
Table showing the IRIS battery life as a function of the number of gestures performed per hour. At 10 gestures per hour, the battery life is 16.6 hours for continuous usage and 32.9 hours for a full day's usage and 8 hours of SLEEP (corresponding to a user being away from Home WiFi for 8 hours).  At 30 gestures per hour, the battery life is 15.9 hours for continuous usage and 31.5 hours for a full day's usage and 8 hours of SLEEP.  At 60 gestures per hour, the battery life is 14.9 hours for continuous usage and 29.5 hours for a full day's usage and 8 hours of SLEEP. 


Figure 16
Bar chart showing IRIS classification performance as a function of distance to the smart device. The maximum distances at which IRIS can correctly detect and classify devices are 2.06 meters for the Homepod Mini, 4.47 meters for the blinds, 2.97 meters for the door, 3.45 meters for the lights when off, 5.46 meters for the lights when on, and 4.5 meters for the TV. 


Figure 17 
Six photos arranged in a three by three grid captured by IRIS. The column headings are of device categories. These are, from left to right, blinds, speaker and lights off. Each row shows a sample image of the column device at a given illumination level or lux. The illumination levels increase from top to bottom. The first row of photos are at low illumination and show a sample picture of a blind at 1.1 lux and 2 bounding boxes drawn around lights on the ceiling, a picture of a speaker at 0.7 lux with no bounding box, and a picture of lights at 0.5 lux with no bounding box. The second row is the same scene but at higher lux levels of 2.2, 0.9, and 1.2 lux for the blinds, speakers and lights off respectively. Each image shows a correctly drawn bounding box around the target device. The last row shows the same scene but at 13, 12.2, and 52.8 lux for the blinds, speaker and lights off respectively. All photos show correct bounding boxes drawn around each device. This figure shows how the auto exposure on IRIS assists the object detection in low lighting conditions.



